Quantum Graph-State Synthesis with SAT

In quantum computing and quantum information processing, graph states are a specific type of quantum states which are commonly used in quantum networking and quantum error correction. A recurring problem is finding a transformation from a given source graph state to a desired target graph state using only local operations. Recently it has been shown that deciding transformability is already NP-hard. In this paper, we present a CNF encoding for both local and non-local graph state operations, corresponding to one- and two-qubit Clifford gates and single-qubit Pauli measurements. We use this encoding in a bounded-model-checking set-up to synthesize the desired transformation. Additionally, for a completeness threshold on local transformations, we provide an upper bound on the length of the transformation if it exists. We evaluate the approach in two settings: the first is the synthesis of the ubiquitous GHZ state from a random graph state where we can vary the number of qubits, while the second is based on a proposed 14 node quantum network. We find that the approach is able to synthesize transformations for graphs up to 17 qubits in under 30 minutes.

==> sections/06-Discussion.tex <==
\section{Discussion}
% Summary of results
In this work we presented a Boolean encoding for graph-state synthesis.
We use this encoding in a bounded-model-checking set-up to synthesize transformations using only local operations, a problem which has been shown to be NP-hard~\cite{dahlberg2020how}, even when restricting the target graph to a practically-relevant scenario~\cite{dahlberg2020transforming}.
Our work is applicable to general graphs, while the existing FPT algorithm has such a rapidly growing FPT function, that the authors remark themselves it is not usable in practice~\cite{dahlberg2018transforming}.
Our work is general, in contrast to special cases for which polynomial-time algorithms have been found~\cite{dahlberg2020how,hahn2019quantum} or reachability has been excluded~\cite{hahn2022limitations, jong2023extracting}.

We empirically showed that our method synthesizes transformations for problem instances up to 16 qubits.
In comparison, for transformations under single-qubit Clifford operations only, various properties of equivalence classes have been explored up to 12 qubits~\cite{danielsen2006classification,cabello2011optimal,adcock2020mapping} (for single-qubit Clifford transformations of graph states without measurements, the decidability problem is in P~\cite{bouchet1991efficient,nest2004efficient}, while counting all reachable graphs is \#P-complete~\cite{dahlberg2020counting}).
We showed that our work is extendible to solving graph-state equivalence under multi-qubit Cliffords 
%and single-qubit measurements 
on specified subsets of qubits, for which up to 10 qubits was explored before~\cite{englbrecht2022transformations}%\todo{we should read this paper in more detail}.

Synthesizing optimal Clifford circuits without measurements (closely related to graph-state synthesis under LC + edge flips on any pair of nodes, but without VD) has been tackled with BMC in~\cite{schneider2023sat} up to 26 qubits in under 3 hours.
Without the optimality constraint (e.g. find the shortest circuit) this problem is in P~\cite{aaronson2004improved}, while the complexity with the optimality constraint is unknown.
SAT based techniques have also been applied to quantum circuit equivalence checking for a limited selection of quantum circuits~\cite{yamashita2010fast}.
BMC specifically has been applied to Clifford circuit (without measurements) equivalence checking~\cite{berent2022towards} (a problem that is also in P~\cite{amy2018towards}), and an SMT based approach has been used to transform logical quantum circuits to fit physical quantum-chip layouts~\cite{tan2020optimal}.


% Future work
Future work includes the investigation of possibly more efficient ways to encode the problem.
Specifically in the setting where only local operations (LC+VD) are allowed, i.e. $D = \emptyset$ in \cref{def:gs-reach}, we can make use of the fact that the circuit in \cref{fig:gs-transform-circ} is universal for this setting.
The transition relation would then only allow for LC, and VD would be encoded in the constraint over the target state. % by constraining the target state exclusively over the non-isolated nodes in $G_t$.
Another avenue is to avoid exploring isomorphic graphs~\cite{heule2019optimal,codish2013breaking}.
Additionally, similar to MaxSAT approaches to graph problems~\cite{peruvemba2020maxsat} and quantum circuit synthesis~\cite{schneider2023sat}, a (weighted) MaxSAT encoding could be proposed in which a certain type of operation would be minimized.
%\todo[inline]{and say something about the MaxSAT approach? Has already been used for graphs in e.g. \url{https://link.springer.com/chapter/10.1007/978-3-030-58475-7_28}}
We could also apply BMC to related NP-hard problems~\cite{dahlberg2020transforming}, or apply model-counting techniques~\cite{gomes2021model} to the \#P-complete problem from~\cite{dahlberg2020counting}.

%Extensions of our work with more expressive languages include model-counting techniques~\cite{gomes2021model} for the \#P-complete problem from~\cite{dahlberg2020counting}, to opt for integer-linear programming~\cite{eiben2018unary}.

%\todo[inline]{maybe something with smt solvers?}

% Other future work?

% Maybe reference this parity problem \url{https://www.sciencedirect.com/science/article/pii/S0166218X06004586#aep-enunciation-id10} in the discussion?


==> sections/Related-Work.tex <==
\section{Related work}
%The transformation of graph states has been extensively studied from the theory standpoint~\cite{nest2004graphical, nest2005thesis, hein2004multiparty,ji2008lulc,hein2006entanglement}.
%, expressing graph-state operations as transformations on the assocated graphs
When only considering single-qubit Clifford operations, it has been shown that reachability for graph states is decidable in 
Various properties of equivalence classes in graph states under LC have been explored up to 12 qubits
%In addition, the structure of the relationship between graph states under LC has been explored numerically up to 9 qubits~\cite{adcock2020mapping}.
Synthesizing Clifford circuits without measurements which produce some target state (closely related to graph state synthesis under LC + edge flips on any pair of nodes, but without VD) has been tackled with BMC in~\cite{schneider2023sat} up to 26 qubits in under 3 hours. Without the optimality constraint (e.g. find the shortest circuit) this problem is in P~\cite{aaronson2004improved}, while the complexity with the optimality constraint is unknown.

When extending the allowed operations with vertex deletions, deciding reachability becomes NP-complete~\cite{dahlberg2018transforming}, even in various scenarios when the target graph state is restricted to often-used quantum states~\cite{dahlberg2020transforming}.
An algorithm to find a transformation from a source to a target graph which is fixed-parameter tractable in the rank-width of $G_s$ and the number of non-isolated vertices in $G_t$ is given in~\cite{dahlberg2018transforming}, but according to the authors is not practical due to bad prefactors.
For special cases, polynomial time algorithms have been found~\cite{dahlberg2020how,hahn2019quantum} or reachability has been excluded~\cite{hahn2022limitations, jong2023extracting}.

%is given in~\cite{dahlberg2020how} but it only works for graphs of rank-width one.
%Polynomial time algorithms also exist for other special cases, such as the synthesis of 3-qubit GHZ states from arbitrary source graphs~\cite{hahn2019quantum}, distance-hereditary graphs~\cite{dahlberg2020how}.
%Reachability has been excluded for some scenarios


%, as well as approximation algorithms~\cite{meignant2019distributing}.
%We do not go into transformations of graph states under more general unitaries than Cliffords, also an active field~\cite{ji2008lulc, hein2004multiparty, englbrecht2020symmetries}.

%TODO reachability LC+VD
%\begin{itemize}
%\item hahn2022limitations \cite{hahn2022limitations}
%\item jong2023extracting \cite{jong2023extracting}
%\item elliott2008graphicalclifford \cite{elliott2008graphicalclifford}
%\item elliott2010graphicalmeasurement \cite{elliott2010graphicalmeasurement}
%\end{itemize}
%TODO: Synthesis
%\begin{itemize}
%\item meignant2019distributing \cite{meignant2019distributing}
%\item mhalla2004complexity \cite{mhalla2004complexity}
%\item vijayan2022compilation \cite{vijayan2022compilation}
%\item lee2023graphtheoretical \cite{lee2023graphtheoretical}
%\end{itemize}
%TODO: multi-qubit equivalence
%\begin{itemize}
%\item englbrecht2022transformations \cite{englbrecht2022transformations} (already referenced in paper)
%\item molengraaf2019thesis \cite{molengraaf2019thesis}
%\item adcock2018hard \cite{adcock2018hard}
%\item joo2011edge \cite{joo2011edge}
%\end{itemize}
%TODO: extend to general local unitaries instead of just Cliffords
%\begin{itemize}
%\item nest2004local \cite{nest2004local}
%\item nest2005local \cite{nest2005local}
%\item ji2008lulc \cite{ji2008lulc}
%\item gross2007lulc \cite{gross2007lulc}
%\item sarvepalli2010local \cite{sarvepalli2010local}
%\item tsimakuridze2017graph \cite{tsimakuridze2017graph}
%\item tzitrin2018local \cite{tzitrin2018local}
%\item hein2006entanglement \cite{hein2006entanglement}  (already referenced in paper)
%\item hein2004multiparty \cite{hein2004multiparty}
%\item cabello2009entanglement \cite{cabello2009entanglement}
%\item englbrecht2020symmetries \cite{englbrecht2020symmetries}
%\end{itemize}
%TODO: Applications
%\begin{itemize}
%\item guo2016graph \cite{guo2016graph}
%\end{itemize}
%TODO: Misc
%\begin{itemize}
%\item anders2006fast \cite{anders2006fast}
%\item fischer2020distributing \cite{fischer2020distributing}
%\item hein2006entanglement \cite{hein2006entanglement} (already referenced in paper)
%\item eisert2006multiparticle \cite{eisert2006multiparticle}
%\item zhao2016fast \cite{zhao2016fast}
%\item hwang2015relation \cite{hwang2015relation}
%\item nest2007classical \cite{nest2007classical}
%\item hein2004multiparty \cite{hein2004multiparty}
%\item danos2007measurement \cite{danos2007measurement}
%\item mannalath2023entanglement \cite{mannalath2023entanglement}
%\item nest2005finite \cite{nest2005finite}
%\item nest2005invariants \cite{nest2005invariants}
%\item morley2018loss \cite{morley2018loss}
%\end{itemize}

%It was shown before~\cite{vandennest2004efficient} that when only restricting to single-qubit Clifford gates (i.e. without measurement), the graph-state reachability problem is decidable in P.
%Since then, graph-state reachability under single-qubit Cliffords has received ample attention, focusing on 
%completely mapping out reachability up to 9 qubits~\cite{adcock},
%specific graphs~\cite{jarnpaper},
%... \todo{add more}.

%When including measurements, however, the reachability problem becomes NP-complete~\cite{dahlberg2020transform}, even in various scenarios when the target graph state is restricted to often-used quantum states.
%Although we might therefore not expect to find a polynomial-time algorithm for the general decidability problem, an algorithm was found which is fixed-parameter tractable in the rank-width of the input graph~\cite{dahlberg2020transform}.
%However, as also mentioned in~\cite{dahlberg2020transform}, this FPT algorithm is not practical due to bad prefactors.

%Graph-state reachability using multi-qubit Cliffords but without measurements has been done using bounded model checking on a binary-matrix formalism (no graphs) in \cite{schneider2023sat}.
%In~\cite{englbrecht2022transformations}, the general multi-qubit setting was considered.
%Reachability under general quantum gates is a separate field~\cite{} that is out of scope for this work.

%Finally, we note that since we include measurements, the problem we tackle here is of a different kind than considering only (multi-qubit) Clifford gates, which 
%First, an efficient algorithm, based on graph theory, already existed before for the single-qubit Clifford case without measurements, rendering the need for a model checking approach unnecessary.
%Moreover, it is not clear whether the binary-matrix approach of \cite{schneider2022sat} will be feasible in practice when adding single-qubit measurements, since doing so lifts the problem from P to NP.

%When restricting this set of operations to only local complementations (corresponding single qubit Clifford gates), a polynomial time algorithm which decides reachability (and constructs a sequence of operations) exists~\cite{vandennest2004efficient}. However, when considering both local complementations and vertex deletions (corresponding to single-qubit measurements) the reachability problem has been shown to be NP-complete~\cite{dahlberg2020transform}.

%\todo[inline]{
%(?) Mention Wille Cliff SAT paper here?
%}

